Estimating Heterogeneous Treatment Effects in Residential Demand Response

We evaluate the causal effect of hour-ahead price interventions on the reduction in residential electricity consumption using a data set from a large-scale experiment on 7,000 households in California. By estimating user-level counterfactuals using time-series prediction, we estimate an average treatment effect of ~0.10 kWh (11%) per intervention and household. Next, we leverage causal decision trees to detect treatment effect heterogeneity across users by incorporating census data. These decision trees depart from classification and regression trees, as we intend to estimate a causal effect between treated and control units rather than perform outcome regression. We compare the performance of causal decision trees with a simpler, yet more inaccurate k-means clustering approach that naively detects heterogeneity in the feature space, confirming the superiority of causal decision trees. Lastly, we comment on how our methods to detect heterogeneity can be used for targeting households to improve cost efficiency.

==> Sections/Adaptive_Targeting.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% This is Adaptive_Targeting.tex (part of DR_RCT.tex)
% author: Datong Zhou
% last edited: July 7, 2017
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% !TEX root = ../DR_RCT.tex
\section{Effect of Adaptive Targeting}
\label{sec:adaptive_targeting}

\subsection{Targeting Assignment Algorithm}
Recall the model for the estimation of user-level counterfactuals \eqref{eq:observation_outcome_model}, here repeated for convenience:
\begin{align}\label{eq:observation_outcome_model_rep}
y_{it} = f_i(\mathbf{x}_{it}) + D_{it}\cdot\beta_{it}(\mathbf{x}_{it}) + \varepsilon_{it}.
\end{align}
Also, recall that an estimate of user $i$'s ITE $\hat{\beta}_i$ is obtained by marginalizing $\lbrace \hat{\beta}_{it}\rbrace_{t\in\mathcal{T}_i}$. We now want to define a targeting strategy $g(\beta_i, \boldsymbol{\beta}_{-i}) = g(\boldsymbol{\beta})$ that maps ITE estimates $\boldsymbol{\beta}$ to treatment assignments (we abuse notation and write $\boldsymbol{\beta}$ in lieu of $\boldsymbol{\hat{\beta}}$).

Defining $\boldsymbol{\beta}_i := \lbrace \beta_{it} \rbrace_{t\in\mathcal{T}_i} \in \mathbb{R}^{|\mathcal{T}_i|}$ and $\boldsymbol{r}_i := \lbrace r_{it} \rbrace_{t\in\mathcal{T}_i} \in \mathbb{R}^{|\mathcal{T}_i|}$, i.e. the collection of all one-sample treatment effects and incentive levels, we define targeting to be efficient if
\begin{align}
\mathbb{E}_{i\in\mathcal{I}}[h(\boldsymbol{\beta}_i, \boldsymbol{r}_i)~|~g(\beta_i)] &> \mathbb{E}_{i\in\mathcal{I}}[h(\boldsymbol{\beta}_i, \boldsymbol{r}_i)~|~D_i],
\end{align}
where $h(\cdot, \cdot) = \mathbb{R}^{|\mathcal{T}_i|} \times \mathbb{R}^{|\mathcal{T}_i|} \to \mathbb{R}$ maps the estimated one-sample treatment effects $\boldsymbol{\beta}_i$ and incentive levels $\boldsymbol{r}_i$ to a desired (scalar) targeting metric. $D_i$ is random assignment to reward levels. In other words, the marginalization of user-level metrics shall outperform random assignment in terms of a scalar metric. The idea for Phase 2 targeting is simple:
\begin{itemize}
\item Right after Phase 1, estimate a set of ITEs $\lbrace\hat{\beta}_{i}\rbrace_{i\in\mathcal{I}}$.
\item Right before Phase 2 begins, analyze the distribution of estimated ITEs, define a targeting metric $h$, and then design the targeting strategy (or assignment strategy) $g$ for subsequent Phase 2 interventions.
\end{itemize}

\subsection{Targeting Assignment Strategy and Metrics}
We use a simple partitioning methodology that assigns users from Phase 1 to two different targeted groups in Phase 2. More specifically, let $g(\beta_i, \boldsymbol{\beta}_{-i})$ be defined as follows:
\begin{align}\label{eq:targeting_partitioning_strategy}
g(\beta_i, \boldsymbol{\beta}_{-i}) =
\begin{cases}
H &\mbox{if } \beta_i > \text{median}(\lbrace \beta_i \rbrace_{i\in\mathcal{I}}) \\ 
L &\mbox{if } \beta_i \leq \text{median}(\lbrace \beta_i \rbrace_{i\in\mathcal{I}})
\end{cases},
\end{align}
where $H = \text{unif}\lbrace 1, 3 \rbrace$ and $L = \text{unif}\lbrace 0.05, 0.10, 0.25 \rbrace$, that is, users in $H$ ($L$) receive high (low) incentive levels during Phase 2. More concretely, the 50\% of the largest (smallest) reducers from Phase 1 receive low (high) incentives in Phase 2. This targeting scheme appears to be a double-edged sword: 
On the one hand, the DRP pays less money to large reducers and also achieves larger reductions for previously small reducers, increasing the desired ratio. On the other hand, previously large reducers now reduce less (in response to smaller rewards) and previously small reducers are paid more money for increased reductions, thereby counteracting the desired goal. However, the latter factors are dominated by the gains from the former ones, as we show in Section \ref{sec:targeting_results}.

From the perspective of the DR Provider, the goal is to maximize the reduction per dollar paid to the users, which is achieved by either minimizing the payout and/or maximizing users' reductions. Accordingly, we define the targeting metric $h_1(\boldsymbol{\beta}_i, \boldsymbol{r}_i)$ to be
\begin{align}\label{eq:targeting_metric_v1}
h_1(\boldsymbol{\beta}_i, \boldsymbol{r}_i) = \boldsymbol{\beta}_i^\top \mathbf{1} / (\boldsymbol{\beta}_i^\top \boldsymbol{r}_i),
\end{align}
that is, the sum of event-wise reductions $\boldsymbol{\beta}_i^\top \mathbf{1}$ divided by the payments made to user $i$, $\boldsymbol{\beta}_i^\top \boldsymbol{r}_i$. Alternatively, to take varying incentive levels offered to the user into account, we can also extend \eqref{eq:targeting_metric_v1} as follows:
\begin{align}\label{eq:targeting_metric_v2}
h_2(\boldsymbol{\beta}_i, \boldsymbol{r}_i) = \frac{\boldsymbol{\beta}_i^\top \mathbf{1}}{\boldsymbol{\beta}_i^\top \boldsymbol{r}_i}\bigg/ \frac{\boldsymbol{r}_i^\top \mathbf{1}}{|\boldsymbol{r}_i|} = \frac{h_2 |\boldsymbol{r}_i|}{\boldsymbol{r}_i^\top \mathbf{1}}.
\end{align}
That is, we normalize $h_1$ defined in \eqref{eq:targeting_metric_v1} by the average incentive level offered to user $i$, as higher incentive levels offered to users are likely to elicit larger treatment effects.

\subsection{Practical Considerations}
Users are transitioned into Phase 2 on a weekly basis. That is, for a particular week, all users who have reached 90 days of age in Phase 1 form the current weekly cohort, which is \textit{randomly} split into a non-targeted group $\overline{\mathcal{T}}$, whose users continue to receive all incentive levels, and a targeted group $\mathcal{T}$ of equal size (ties are broken randomly). $\overline{\mathcal{T}}$ acts as a control group against which we benchmark the metrics \eqref{eq:targeting_metric_v1} and \eqref{eq:targeting_metric_v2}. Users in $\mathcal{T}$ are then assigned to $H$ and $L$ according to \eqref{eq:targeting_partitioning_strategy}.

\subsection{Results of Adaptive Targeting}\label{sec:targeting_results}
To obtain targeting metrics averaged across users in the targeted and non-targeted groups, we marginalize \eqref{eq:targeting_metric_v1} and \eqref{eq:targeting_metric_v2} across targeted and non-targeted users to obtain 
\begin{itemize}
\item $H_1^{\mathcal{T}}$ and $H_1^{\overline{\mathcal{T}}}$, i.e. \eqref{eq:targeting_metric_v1} for all targeted/non-targeted users
\item $H_2^{\mathcal{T}}$ and $H_2^{\overline{\mathcal{T}}}$, i.e. \eqref{eq:targeting_metric_v2} for all targeted/non-targeted users
\end{itemize}

Table \ref{tab:targeting_metrics} shows the results.
\begin{table}[hbtp]
\vspace*{0.1cm} 
\centering
\begin{tabular}{c|cccccc}
\toprule
\multicolumn{7}{c}{Targeting Metrics for Phase 2} \\
\hline
Estimator & $H_1^{\mathcal{T}}$ & $H_1^{\overline{\mathcal{T}}}$ & $H_2^{\mathcal{T}}$ & $H_2^{\overline{\mathcal{T}}}$ & $\text{CATE}_{\mathcal{T}}$ & $\text{CATE}_{\overline{\mathcal{T}}}$  \\
\hline
BL & $1.411$ & $1.044$ & $1.273$ & $1.070$ & $-0.0743$ & $-0.0861$  \\
L2 & $2.934$ & $1.070$ & $2.655$ & $1.096$ & $-0.0441$ & $-0.0580$  \\
OLS & $2.684$ & $1.069$ & $2.429$ & $1.096$ & $-0.0484$ & $-0.0628$  \\
RF & $2.549$ & $1.085$ & $2.306$ & $1.112$ & $-0.0464$ & $-0.0609$  \\
\bottomrule
\end{tabular}
\vspace{0.1cm}
\caption{Targeting Results for 2,733 users between June 29, 2017 - December 31, 2017. $[H_1] = \frac{\text{kWh}}{\text{USD}}$, $[H_2] = \frac{\text{kWh}^2}{\text{USD}^2}$, $[\text{CATE}] = \text{kWh}$.}
\label{tab:targeting_metrics}
\vspace*{-0.03cm} 
\end{table}
RF predicts a difference of $H_1^{\mathcal{T}} - H_1^{\overline{\mathcal{T}}} \approx 1.464\frac{\text{kWh}}{\text{USD}}$, or an increase of $\approx 135\%$. That is, the targeting mechanism is capable of achieving the same reduction for the targeted as for the non-targeted group with just $\approx 43\%$ of the payout. If we normalize $H_1$ with the average reward offered, RF predicts a difference of $H_2^{\mathcal{T}} - H_2^{\overline{\mathcal{T}}} \approx 1.194\frac{\text{kWh}}{\text{USD}}$, which is an increase of $\approx 107\%$.

Additionally, observe that the absolute value of the CATE among targeted ($|\text{CATE}_{\mathcal{T}}|$) users is smaller than for non-targeted users ($|\text{CATE}_{\overline{\mathcal{T}}}|$), which indicates that the extent to which low-targeted users (large reducers in Phase 1) reduce their reductions dominates the increase in reduction among high-targeted users (small reducers in Phase 2). However, this net reduction of willingness to temporarily reduce electricity consumption is greatly dominated by the assignment of high (low) rewards to low (large) reducers in Phase 1, which explains the $135\%$ and $107\%$ increase of the $H_1$ and $H_2$ metrics, respectively.

==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->,#1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->,#1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


